Asymptotic Theory of Eigenvectors for Latent Embeddings with Generalized Laplacian Matrices

Laplacian matrices are commonly employed in many real applications, encoding the underlying latent structural information such as graphs and manifolds. The use of the normalization terms naturally gives rise to random matrices with dependency. It is well-known that dependency is a major bottleneck of new random matrix theory (RMT) developments. To this end, in this paper, we formally introduce a class of generalized (and regularized) Laplacian matrices, which contains the Laplacian matrix and the random adjacency matrix as a specific case, and suggest the new framework of the asymptotic theory of eigenvectors for latent embeddings with generalized Laplacian matrices (ATE-GL). Our new theory is empowered by the tool of generalized quadratic vector equation for dealing with RMT under dependency, and delicate high-order asymptotic expansions of the empirical spiked eigenvectors and eigenvalues based on local laws. The asymptotic normalities established for both spiked eigenvectors and eigenvalues will enable us to conduct precise inference and uncertainty quantification for applications involving the generalized Laplacian matrices with flexibility. We discuss some applications of the suggested ATE-GL framework and showcase its validity through some numerical examples.

==> name.tex <==
For any $z\in I_k$, we have that w.h.p.,
\begin{align}\label{eq:spiked eigenvalue subtraction 1}
\begin{split}
    \bG(z)=&\frac{1}{\bcW-(\bL/\bLambda)^{-\alpha}z}\\
    =&-\frac{1}{(\bL/\bLambda)^{2\alpha}z}\frac{1}{1-\bcW(\bL/\bLambda)^{-2\alpha}z^{-1}}\\
    =&-\frac{1}{(\bL/\bLambda)^{2\alpha}z}\left(1+\bcW(\bL/\bLambda)^{-2\alpha}z^{-1}+\bcW(\bL/\bLambda)^{-2\alpha}\bcW(\bL/\bLambda)^{-2\alpha}z^{-2}\right)+O(|\delta_k|^{-4})\\
    =&-(\bL/\bLambda)^{-2\alpha}z^{-1}-(\bL/\bLambda)^{-2\alpha}\bcW(\bL/\bLambda)^{-2\alpha}z^{-2}-\bcW^2z^{-3}+O\left(|\delta_k|^{-4}+\frac{\xi}{q|\delta_k|^3}\right)\\
    =&-z^{-1}\bA(z)+O\left(|\delta_k|^{-4}+\frac{\xi}{q|\delta_k|^3}\right),
\end{split}
\end{align}
and  w.h.p. that
\begin{align}\label{eq:spiked eigenvalue subtraction 2}
\begin{split}
    &\bv_k^\top\bG(\hdelta_k)\bV_{-k}\frac{1}{\bDelta^{-1}_{-k}+\bV_{-k}^\top\bG(\hdelta_k)\bV_{-k}}\bV_{-k}^\top\bG(\hdelta_k)\bv_k\\
    \lesssim&\left(\frac{1}{|\delta_k|^3}+\frac{\sqrt K\xi}{q|\delta_k|}\bigg(\frac{1}{|\delta_k|}+\frac{\xi}{q}+\|\bV\|_{\max}\bigg)\right)^2|\delta_k|\\
    \lesssim&\frac{1}{|\delta_k|}\left(\frac{1}{|\delta_k|^4}+\frac{K\xi^2}{q^2}\left(\frac{1}{|\delta_k|^2}+\frac{\xi^2}{q^2}+\|\bV\|_{\max}^2\right)\right).
\end{split}
\end{align}
\begin{comment}
\begin{align}\label{eq:spiked eigenvalue subtraction 2}
\begin{split}
    &\bv_k^\top\bG(\hdelta_k)\bV_{-k}\frac{1}{\bDelta^{-1}_{-k}+\bV_{-k}^\top\bG(\hdelta_k)\bV_{-k}}\bV_{-k}^\top\bG(\hdelta_k)\bv_k\\
    =&\hdelta_k^{-2}\bv_k^\top\bA(\hdelta_k)\bV_{-k}^\top\frac{1}{\bDelta_{-k}^{-1}-\bV_{-k}^\top\bG(\hdelta_k)\bV_{-k}}\bV_{-k}\bA(\hdelta_k)\bv_k+O\left(\left(\frac{1}{|\delta_k|^{4}}+\frac{\xi}{q|\delta_k|^3}\right)\left(\frac{\sqrt K\xi\psi_n}{q}+\frac{1}{|\delta_k|^2}\right)\right)\\
    =&\hdelta_k^{-2}\bv_k^\top\bA(\hdelta_k)\bV_{-k}^\top\frac{1}{\bDelta_{-k}^{-1}+\hdelta_k^{-1}\bV_{-k}^\top\bA(\hdelta_k)\bV_{-k}}\bV_{-k}\bA(\hdelta_k)\bv_k+O\left(\left(\frac{1}{|\delta_k|^{4}}+\frac{\xi}{q|\delta_k|^3}\right)\left(\frac{\sqrt K\xi\psi_n}{q}+\frac{1}{|\delta_k|^2}\right)\right)\\
    =&t_k^{-2}\bv_k^\top\bA(t_k)\bV_{-k}^\top\frac{1}{\bDelta_{-k}^{-1}+t_k^{-1}\bV_{-k}^\top\bA(t_k)\bV_{-k}}\bV_{-k}\bA(t_k)\bv_k\\
    &+O\left(\left(\frac{1}{|\delta_k|^{4}}+\frac{\xi}{q|\delta_k|^3}+\frac{|t_k-\hdelta_k|}{|\delta_k|^2}\right)\left(\frac{\sqrt K\xi\psi_n}{q}+\frac{1}{|\delta_k|^2}\right)\right)
\end{split}
\end{align}
\end{comment}
Substitute (\ref{eq:spiked eigenvalue subtraction 1}), (\ref{eq:spiked eigenvalue subtraction 2}) and (\ref{eqn:t_k-gamma_k 2}) into (\ref{eqn:t_k-gamma_k 1}), we get w.h.p.
\begin{align}\label{eq:eigenvalue expansion 1}
\begin{split}
    &\bv_k^\top(-\hdelta_k^{-1}\bA(\hdelta_k)-\bUpsilon(t_k))\bv_k\\
    \lesssim&\frac{1}{|\delta_k|}\left(\frac{1}{|\delta_k|^4}+\frac{K\xi^2}{q^2}\left(\frac{1}{|\delta_k|^2}+\frac{\xi^2}{q^2}+\|\bV\|_{\max}^2\right)\right)+\frac{1}{|\delta_k|^5}+\frac{1}{|\delta_k|^4}+\frac{\xi}{q|\delta_k|^3}+\frac{|t_k-\hdelta_k|}{|\delta_k|^2}\left(\frac{\sqrt K\xi\psi_n}{q}+\frac{1}{|\delta_k|^2}\right)\\
    \lesssim&\frac{1}{|\delta_k|^4}+\frac{\xi}{q|\delta_k|^3}+\frac{K\xi^2}{q^2|\delta_k|}\left(\frac{\xi^2}{q^2}+\|\bV\|_{\max}^2\right)+\frac{|t_k-\hdelta_k|}{|\delta_k|^2}\left(\frac{\sqrt K\xi\psi_n}{q}+\frac{1}{|\delta_k|^2}\right)
\end{split}
\end{align}
which leads to w.h.p.
\begin{align}
\begin{split}
    t_k^{-1}-\hdelta_k^{-1}=&\hdelta_k^{-1}\bv_k^\top((\bL/\bLambda)^{-2\alpha}-\bI+\hdelta_k^{-1}(\bL/\bLambda)^{-2\alpha}\bcW(\bL/\bLambda)^{-2\alpha}+\hdelta_k^{-2}\bcW^2)\bv_k\\
    &+\bv_k^\top(t_k^{-1}+\bUpsilon(t_k))\bv_k\\
    &+O\left(\frac{1}{|\delta_k|^4}+\frac{\xi}{q|\delta_k|^3}+\frac{K\xi^2}{q^2|\delta_k|}\left(\frac{\xi^2}{q^2}+\|\bV\|_{\max}^2\right)+\frac{|t_k-\hdelta_k|}{|\delta_k|^2}\left(\frac{\sqrt K\xi\psi_n}{q}+\frac{1}{|\delta_k|^2}\right)\right)
\end{split}
\end{align} 
and w.h.p.
\begin{align}
\begin{split}
    \hdelta_k-t_k=&t_k\bv_k^\top((\bL/\bLambda)^{-2\alpha}-\bI+t_k^{-1}(\bL/\bLambda)^{-2\alpha}\bcW(\bL/\bLambda)^{-2\alpha}+t_k^{-2}\bcW^2)\bv_k\\
    &+t_k^2\bv_k^\top(t_k^{-1}+\bUpsilon(t_k))\bv_k\\
    &+O\left(\frac{1}{|\delta_k|^2}+\frac{\xi}{q|\delta_k|}+\frac{K\xi^2|\delta_k|}{q^2}\left(\frac{\xi^2}{q^2}+\|\bV\|_{\max}^2\right)+{|t_k-\hdelta_k|}\left(\frac{\sqrt K\xi\psi_n}{q}+\frac{1}{|\delta_k|}\right)\right).
\end{split}
\end{align}
To begin with, we deal with the first term, note that from Taylor expansion, we have w.h.p.
\begin{align}
\begin{split}
    \bv_k^\top((\bL/\bLambda)^{-2\alpha}-\bI)\bv_k=&\bv_k^\top\left(-2\alpha\frac{\bL-\bLambda}{\bLambda}+\alpha(2\alpha+1)\frac{(\bL-\bLambda)^2}{\bLambda^2}\right)\bv_k+O\left(\frac{\xi^3}{q^3}\right),
\end{split}
\end{align}
while for the quadratic term, we have
\begin{align}
\begin{split}
    &\mathbb E\bv_k^\top\frac{(\bL-\bLambda)^2}{\bLambda^2}\bv_k\\
    =&q^{-2}\sum_{i\in[n]}\mathbb E\left(\sum_{j\in[n]}W_{ij}+\frac{\tau}{n}\sum_{l,j\in[n]}W_{lj}\right)^2\Lambda^{-2}_iv_k(i)^2\\
    =&q^{-2}\sum_{i\in[n]}\left((1+\tau/n)^2s_{ii}+(1+2\tau/n)^2\sum_{j}^{(i)}s_{ij}+\frac{4\tau^2}{n^2}\sum_{j,l}^{(i)}(1+\delta_l^j)^{-2}s_{lj}\right)\Lambda^{-2}_iv_k(i)^2\\
    =&q^{-2}\sum_{i,j\in[n]}s_{ij}\Lambda_i^{-2}v_k(i)^2+O\left(\frac{1}{q^2n}\right),
\end{split}
\end{align}
\begin{align}
\begin{split}
    \mathbb E\left(\bv_k^\top\frac{(\bL-\bLambda)^2}{\bLambda^2}\bv_k\right)^2
    =q^{-2}\sum_{i\in[n]}\mathbb E\left(\sum_{j\in[n]}W_{ij}+\frac{\tau}{n}\sum_{l,j\in[n]}W_{lj}\right)^2\Lambda^{-2}_iv_k(i)^2\bv_k^\top\frac{(\bL-\bLambda)^2}{\bLambda^2}\bv_k
\end{split}
\end{align}
note that for $\{i,j\}\neq\{l,s\}$, we have w.h.p.
\begin{align}
\begin{split}
    \mathbb E W_{ij}W_{ls}\bv_k^\top\frac{(\bL-\bLambda)^2}{\bLambda^2}\bv_k=&s_{ij}\mathbb EW_{ls}\frac{\partial \bv_k^\top\frac{(\bL-\bLambda)^2}{\bLambda^2}\bv_k}{\partial W_{ij}}+r_{ij}\lesssim\frac{\|\bv_k\|_\infty^2}{q^2n}(n^{-1+|\{i,j\}\cap\{l,s\}|}+q^{-1})
\end{split}
\end{align}
where
\[
    r_{ij}\lesssim\mathbb E|W_{ij}|^3\frac{\|\bv_k\|^2_\infty}{q^2}\lesssim\frac{\|\bv_k\|^2_\infty}{q^3n},
\]
and we also estimate that w.h.p.
\begin{align}
\begin{split}
    \mathbb EW_{ij}^2\bv_k^\top\frac{(\bL-\bLambda)^2}{\bLambda^2}\bv_k=&s_{ij}\mathbb E\bv_k^\top\frac{(\bL-\bLambda)^2}{\bLambda^2}\bv_k+O\left(\|\bv_k\|^2_\infty(\mathbb E|W_{ij}|^4-s_{ij}^2)\right)\\
    =&s_{ij}\mathbb E\bv_k^\top\frac{(\bL-\bLambda)^2}{\bLambda^2}\bv_k+O\left(\frac{\|\bv_k\|_\infty^2}{q^2n}\right).
\end{split}
\end{align}
Now we can calculate that w.h.p.
\begin{align}
\begin{split}
    \mathbb E\left(\bv_k^\top\frac{(\bL-\bLambda)^2}{\bLambda^2}\bv_k\right)^2=&q^{-2}\sum_{i,j\in[n]}s_{ij}\Lambda_i^2v_k(i)^2\mathbb E\bv_k^\top\frac{(\bL-\bLambda)^2}{\bLambda^2}\bv_k+O\left(\frac{n\|\bv_k\|^2_\infty}{q^4}+\frac{1}{q^4n^2}\right)\\
    =&\left(\mathbb E\bv_k^\top\frac{(\bL-\bLambda)^2}{\bLambda^2}\bv_k\right)^2+O\left(\frac{n\|\bv_k\|^2_\infty}{q^4}+\frac{1}{q^4n^2}\right)
\end{split}
\end{align}
which leads to
\begin{align}
    \var\left(\bv_k^\top\frac{(\bL-\bLambda)^2}{\bLambda^2}\bv_k\right)\lesssim\frac{n\|\bv_k\|^2_\infty}{q^4}+\frac{1}{q^4n^2}.
\end{align}
For the second term, we have
\begin{align}
\begin{split}
    \bv_k^\top(\bL/\bLambda)^{-2\alpha}\bcW(\bL/\bLambda)^{-2\alpha}\bv_k=&\bv_k^\top\bcW\bv_k-2\alpha\bv_k^\top\frac{\bL-\bLambda}{\bLambda}\bcW\bv_k-2\alpha\bv_k^\top\bcW\frac{\bL-\bLambda}{\bLambda}\bv_k+O\left(\frac{\xi^2}{q^2}\right)\\
    =&\bv_k^\top\bcW\bv_k-4\alpha\bv_k^\top\frac{\bL-\bLambda}{\bLambda}\bcW\bv_k+O\left(\frac{\xi^2}{q^2}\right),
\end{split}
\end{align}
we calculate
\begin{align}
\begin{split}
    \mathbb E\bv_k^\top\frac{\bL-\bLambda}{\bLambda}\bcW\bv_k=&q^{-1}\sum_{i,j\in[n]}v_k(i)v_k(j)\Lambda_i^{-1}\mathbb E\left(\sum_{l\in[n]}W_{il}+\frac{\tau}{n}\sum_{l,s\in[n]}W_{ls}\right)\baW_{ij}\\
    =&q^{-1}\sum_{i,j\in[n]}v_k(i)v_k(j)\Lambda_i^{-1-\alpha}\Lambda_j^{-\alpha}(1+2\tau n^{-1}(1+\delta_i^j)^{-1})s_{ij}\\
    =&q^{-1}\sum_{i,j\in[n]}v_k(i)v_k(j)\Lambda_i^{-1-\alpha}\Lambda_j^{-\alpha}s_{ij}+O\left(\frac{1}{qn}\right),
\end{split}
\end{align}
\begin{align}
\begin{split}
    &\mathbb E\left(\bv_k^\top\frac{\bL-\bLambda}{\bLambda}\bcW\bv_k\right)^2\\
    =&q^{-1}\sum_{i,j\in[n]}v_k(i)v_k(j)\Lambda_i^{-1}\mathbb E\left(\sum_{l\in[n]}W_{il}+\frac{\tau}{n}\sum_{l,s\in[n]}W_{ls}\right)\baW_{ij}\bv_k^\top\frac{\bL-\bLambda}{\bLambda}\bcW\bv_k.
\end{split}
\end{align}
From the cumulant expansion formula we have that for $\{i,j\}\neq\{l,s\}$,
\begin{align}
\begin{split}
    \mathbb EW_{ls}W_{ij}\bv_k^\top\frac{\bL-\bLambda}{\bLambda}\bcW\bv_k=&s_{ij}\mathbb EW_{ls}\frac{\partial\bv_k^\top\frac{\bL-\bLambda}{\bLambda}\bcW\bv_k}{\partial W_{ij}}+\frac{\kappa_3(W_{ij})}{2}\mathbb E W_{ls}\frac{\partial^2\bv_k^\top\frac{\bL-\bLambda}{\bLambda}\bcW\bv_k}{\partial^2 W_{ij}}\\
    \lesssim&\frac{\|\bv_k\|_\infty^2}{q}n^{-3+|\{i,j\}\cap\{l,s\}|}
\end{split}
\end{align}
where the error term
We also have
\begin{align}
\begin{split}
    \mathbb EW_{ij}^2\bv_k^\top\frac{\bL-\bLambda}{\bLambda}\bcW\bv_k=&s_{ij}\mathbb E\bv_k^\top\frac{\bL-\bLambda}{\bLambda}\bcW\bv_k+O\left(\frac{\|\bv_k\|^2_\infty(\mathbb E W_{ij}^4-s_{ij}^2)}{q}\right)\\
    =&s_{ij}\mathbb E\bv_k^\top\frac{\bL-\bLambda}{\bLambda}\bcW\bv_k+O\left(\frac{\|\bv_k\|^2_\infty}{q^3n}\right).
\end{split}
\end{align}
Thus we obtain
\begin{align}
\begin{split}
    \mathbb E\left(\bv_k^\top\frac{\bL-\bLambda}{\bLambda}\bcW\bv_k\right)^2=&q^{-1}\sum_{i,j\in[n]}v_k(i)v_k(j)\Lambda_i^{-1-\alpha}\Lambda_j^{-\alpha}s_{ij}\mathbb E\bv_k^\top\frac{\bL-\bLambda}{\bLambda}\bcW\bv_k\\
    &+O\left(\frac{\|\bv_k\|_\infty^2}{q^2}+\frac{1}{q^2n}\right).
\end{split}
\end{align}
Consider the mean and variance of the third term
\begin{align}
\begin{split}
    \mathbb E\bv_k^\top\bcW^2\bv_k=&\sum_{i,j,l\in[n]}\mathbb Ev_k(i)\baW_{ij}\baW_{jl}v_k(l)\\
    =&\sum_{i,j}v_k(i)^2s_{ij}(\Lambda_i\Lambda_j)^{-2\alpha},
\end{split}
\end{align}
\begin{align}
\begin{split}
    &\mathbb E(\bv_k^\top\bcW^2\bv_k)^2\\
    =&\sum_{i,j,l\in[n]}\mathbb Ev_k(i)\baW_{ij}\baW_{jl}v_k(l)\bv_k^\top\bcW^2\bv_k\\
    =&\sum_{i,j}^{[n]}\sum_{l}^{(i)}v_k(i)v_k(l)\left((\Lambda_i\Lambda_j)^{-2\alpha}s_{ij}\mathbb E\frac{\partial(\baW_{jl}\bv_k^\top\bcW^2\bv_k)}{\partial\baW_{ij}}+r_{ijl}\right)\\
    &+\sum_{i,j}^{[n]}\mathbb Ev_k(i)^2\baW_{ij}^2\bv_k^\top\bcW^2\bv_k\\
    =&\sum_{i,j}^{[n]}\sum_{l}^{(i)}v_k(i)v_k(l)\left((\Lambda_i\Lambda_j)^{-2\alpha}s_{ij}\mathbb E\baW_{jl}\frac{\partial(\bv_k^\top\bcW^2\bv_k)}{\partial\baW_{ij}}+r_{ijl}\right)\\
    &+(\mathbb E\bv_k^\top\bcW^2\bv_k)^2+O\left(\sum_{i,j}^{[n]}|v_k(i)|^2(|v_k(i)|^2+|v_k(j)|^2)(\mathbb E|W_{ij}|^4-s_{ij}^2)\right)
\end{split}
\end{align}
where the error term
\[
    r_{ijl}\lesssim\mathbb E|W_{ij}|^3(v_k(i)^2+v_k(j)^2)\mathbb E|W_{jl}|\lesssim\frac{v_k(i)^2+v_k(j)^2}{qn^{3/2}}.
\]
Thus we obtain
\begin{align}\label{eq:eigenvalue expansion 2}
\begin{split}
    \var(\bv_k^\top\bcW^2\bv_k)\lesssim&\left|\sum_{i,j}^{[n]}\sum_{l}^{(i)}v_k(i)v_k(l)(\Lambda_i\Lambda_j)^{-2\alpha}s_{ij}\mathbb E\baW_{jl}\frac{\partial(\bv_k^\top\bcW^2\bv_k)}{\partial\baW_{ij}}\right|+O\left(\frac{1}{q\sqrt n}+\frac{\|\bv_k\|_\infty^2}{q^2}\right)\\
    \lesssim&\sum_{i,j}^{[n]}\sum_{l}^{(i)}v_k(i)^2v_k(l)^2s_{ij}s_{jl}+O\left(\frac{1}{q\sqrt n}+\frac{\|\bv_k\|_\infty^2}{q^2}\right)\\
    \lesssim&\frac{1}{n}+\frac{1}{q\sqrt n}+\frac{\|\bv_k\|_\infty^2}{q^2}.
\end{split}
\end{align}
Combining (\ref{eq:eigenvalue expansion 1})-(\ref{eq:eigenvalue expansion 2}), we deduce that
\begin{align}
\begin{split}
    \hdelta_k-t_k=&-2\alpha t_k\bv_k^\top\frac{\bL-\bLambda}{\bLambda}\bv_k+\alpha(2\alpha+1)\frac{t_k}{q^2}\sum_{i,j\in[n]}v_k(i)^2\Lambda_i^{-2}s_{ij}+O\left(\frac{|\delta_k|}{q^2n}+\frac{\xi^3|\delta_k|}{q^3}\right)+B_1\\
    &+\bv_k^\top\bcW\bv_k-\frac{2\alpha}{q}\sum_{i,j\in[n]}v_k(i)v_k(j)\Lambda_i^{-1-\alpha}\Lambda_j^{-\alpha}s_{ij}+O\left(\frac{1}{qn}+\frac{\xi^2}{q^2}\right)+B_2\\
    &+\frac{1}{t_k}\sum_{i,j\in[n]}v_k(i)^2(\Lambda_i\Lambda_j)^{-2\alpha}s_{ij}+B_3+t_k^2\bv_k^\top(t_k^{-1}+\bUpsilon(t_k))\bv_k\\
    &+O\left(\frac{1}{|\delta_k|^2}+\frac{\xi}{q|\delta_k|}+\frac{K\xi^2|\delta_k|}{q^2}\left(\frac{\xi^2}{q^2}+\|\bV\|_{\max}^2\right)+{|t_k-\hdelta_k|}\left(\frac{\sqrt K\xi\psi_n}{q}+\frac{1}{|\delta_k|}\right)\right)
\end{split}
\end{align}
w.h.p., where $B_1,B_2,B_3$ are centered random variables satisfying
\begin{align}
    \var B_1&\lesssim \frac{n\|\bv_k\|_\infty^2|\delta_k|^2}{q^4}+\frac{|\delta_k|^2}{q^4n^2},\\
    \var B_2&\lesssim\frac{\|\bv_k\|_\infty^2}{q^2}+\frac{1}{q^2n},\\
    \var B_3&\lesssim\frac{1}{n|\delta_k|^2}+\frac{1}{q\sqrt n|\delta_k|^2}+\frac{\|\bv_k\|_\infty^2}{q^2|\delta_k|^2}.
\end{align}
It remains to obtain the CLT of the linear term
\begin{align}
\begin{split}
    &-2\alpha t_k\bv_k^\top\frac{\bL-\bLambda}{\bLambda}\bv_k+\bv_k^\top\bcW\bv_k\\
    =&-2\alpha t_kq^{-1}\sum_{i\in[n]}\left(\sum_{j\in[n]}W_{ij}+\frac{\tau}{n}\sum_{l,j\in[n]}W_{lj}\right)\Lambda_i^{-1}v_k(i)^2\\
    &+\sum_{i,j\in[n]}v_k(i)v_k(j)(\Lambda_i\Lambda_j)^{-\alpha}W_{ij}\\
    =&\sum_{i\leq j\in[n]}(1+\delta_i^j)^{-1}\left(-\frac{2\alpha t_k}{q}\left(\frac{v_k(i)^2}{\Lambda_i}+\frac{v_k(j)^2}{\Lambda_j}+\frac{2\tau}{n}\sum_{l\in[n]}\Lambda_l^{-1}v_k(l)^2\right)+2v_k(i)v_k(j)(\Lambda_i\Lambda_j)^{-\alpha}\right)W_{ij},
\end{split}
\end{align}
define the variance
\begin{align}
    \sigma_n^2:=\sum_{i\leq j\in[n]}(1+\delta_i^j)^{-2}\left(-\frac{2\alpha t_k}{q}\left(\frac{v_k(i)^2}{\Lambda_i}+\frac{v_k(j)^2}{\Lambda_j}+\frac{2\tau}{n}\sum_{l\in[n]}\Lambda_l^{-1}v_k(l)^2\right)+2v_k(i)v_k(j)(\Lambda_i\Lambda_j)^{-\alpha}\right)^2s_{ij}.
\end{align}
If we have
\begin{align}
    \frac{1}{|\delta_k|^2}+\frac{\xi}{q|\delta_k|}+\frac{K\xi^2|\delta_k|}{q^2}\left(\frac{\xi^2}{q^2}+\|\bV\|_{\max}^2\right)+\frac{|\delta_k|}{q^2n}+\frac{\xi^3|\delta_k|}{q^3}+\frac{1}{qn}+\frac{\xi^2}{q^2}+\sum_{i=1}^3\sqrt{\var B_i}\lesssim\sigma_n,
\end{align}
we would get the CLT of spiked eigenvalue.
